Non-factorizable ribbon Hopf Algebras

Building on the work of Nenciu we provide examples of non-factorizable ribbon Hopf algebras, and introduce a stronger notion of non-factorizability. These algebras are designed to provide invariants of $4$-dimensional $2$-handlebodies up to 2-deformations. We prove that some of the invariants derived from these examples are invariants dependent only on the boundary or on the presentation of the fundamental group of the 2-handlebody.

==> algebra.tex <==
 In this section we study explicit examples of the Nenciu construction. We start with a (not strongly) non-factorizable Hopf algebra, which can be retrieved from Nenciu's construction, and appears in \cite{nenciu_2004} as $E(n)$, first studied in \cite{panaite_oystaeyen_1999}. Here we will refer to it as \textit{symplectic fermions}, after \cite{gainutdinov_runkel_2017}, also appearing in \cite{faitg_gainutdinov_schweigert_2024}.
 \begin{definition}
 \label{SFdef}
     By the \textit{Hopf algebra of symplectic fermions}, $SF_{2n}$ we mean the Hopf algebra generated by $L$ and $Z^\pm_l$, for $k, l=1, \dots, n$, subject to the following relations
    \[
         L^2 = \1, \;\; L Z^\pm_l = - Z^\pm_l L, \;\; \{Z^\pm_l, Z^\pm_k\}=\{Z^\pm_l, Z^\mp_k\}=0.
    \]
    The Hopf structure is defined by
    \[
        \epsilon(L) = 1, \;\; \epsilon(Z^{\pm}_l)= 0,
    \]
    \[
        \Delta(L) = L \otimes L, \;\; \Delta(Z^{\pm}_l) = \1 \otimes Z^{\pm}_l + Z^{\pm}_l \otimes L,
    \]
    \[
        S(L)=L^{-1}=L, \;\; S(Z^{\pm}_l) = -Z^{\pm}_l L.
    \]
    The dimension of the algebra is $2^{2n+1}$. The corresponding Nenciu data is $s=1$, $\mb{m}=m=2$, a tuple with one element and $t=2n$. Thus $\mb{d} = \mb{u} = (1, \dots, 1)^T$ are column vectors whose each row $d_k = 1$ and $u_k = 1$, $k=1, \dots, t$. 
 \end{definition}
\begin{proposition}
    The algebra $SF_{2n}$ of Definition \ref{SFdef} is
    \begin{enumerate}
        \item Unimodular, with two-sided integral element (cointegral)
        \[
            \Lambda := (\1+L)\prod^{n}_{l=1}Z^+_l
            \prod^{n}_{l=1}Z^-_l.
        \]
        and a two-sided integral form defined on the monomial basis by
        \[
            \lambda(\mb{X}^\mb{r} L^v):=
            \begin{cases}
                1 \text{\, if \,} v = 0, \mb{r} = (1, 1,\dots,1) \\
                0 \text{\, otherwise}.
            \end{cases}
        \]
        \item quasitriangular, with the R-matrix defined for the grouplike elements 
        \[
            R_{\mb{z}} := \frac{1}{2}\sum_{v, w \in \Z_2} (-1)^{-vw} L^{w} \otimes L^{v z} = \frac{1}{2}(\1\otimes \1+ \1\otimes L + L\otimes \1 - L\otimes L), 
        \]
        where $z=1$.
        \\The skew-primitive part is 
        \[
            R_{\pmb{\alpha}} := \exp\left(\sum^{t_2}_{l = 1} \alpha_l( Z^+_l \otimes L Z^-_l - Z^-_l \otimes L Z^+_l)\right)
        \]
        for some $\pmb{\alpha}=(\alpha_1, \dots, \alpha_{t_2}) \in \C^{2t_2}$, so that 
        \[
            R = \frac{1}{2}(\1\otimes \1+ \1\otimes L + L\otimes \1 - L\otimes L) \exp\left(\sum^{n}_{l = 1} \alpha_l( Z^+_l \otimes L Z^-_l - Z^-_l \otimes L Z^+_l)\right),
        \]
        \item ribbon, with the ribbon element
        \[
            v:= \exp \left( - 2\sum^{n}_{k = l} \alpha_l Z^+_l Z^-_l  \right).
        \]
        corresponding to the pivotal element $g = L$, which in this example is the only such element available. 
    \end{enumerate}
\end{proposition}
\begin{proof}
    See \cite{panaite_oystaeyen_1999} or \cite{gainutdinov_runkel_2017} in the more general quasi-Hopf algebraic setting.
\end{proof}
We now present examples of the Nenciu construction, exhibiting slightly different properties, but all of them non-factorizable. They can be thought of as generalisations of $SF_{2n}$ with more types of grouplike and nilpotent generators. The proofs of the fact that they are all unimodular, ribbon Hopf algebras are just straightforward applications of the introduced theory, and the required axioms were verified by direct computation.
\begin{example}
\label{ex1}
    Let $H_1$ be the Hopf algebra generated by $K_a$, $X_k$, $Z^{\pm}_l$ for $a=1, 2$, $j, k=1, \dots, t_1$; $ t_1\in 4\N$ and $l, m=1, \dots, t_2$; $t_2\in \N$, subject to the following relations
    \[
         K_a^4 = \1, \;\; K_a X_j = i X_j K_a, \;\; K_1 Z^{\pm}_l = \pm iZ^\pm_l K_1, \;\; K_2 Z^{\pm}_l =   Z^\pm_l K_2,
    \]
    \[
        Z^\pm_l X_k = \mp i X_k Z^\pm_l, \;\;\;  \{X_j, X_k\}= \{Z^{\pm}_l, Z^{\pm}_m\}=\{Z^{\pm}_l, Z^{\mp}_m\} =  0.
    \]
    The Hopf structure is defined by
    \[
        \epsilon(K_a) = 1, \;\; \epsilon(X_k) =\epsilon(Z^{\pm}_l)= 0,
    \]
    \[
        \Delta(K_a) = K_a \otimes K_a, \;\; \Delta(X_k) = \1 \otimes X_k + X_k \otimes K_1 K_2, \;\; \Delta(Z^{\pm}_l) = \1 \otimes Z^{\pm}_l + Z^{\pm}_l \otimes K_1^{\pm 2} K_2^{\mp 1} ,
    \]
    \[
        S(K_a)=K^{-1}_a, \;\; S(X_k) = -X_k (K_1 K_2)^{-1}, \;\; S(Z^{\pm}_l) = -Z^{\pm}_l K_1^{\mp 2} K_2^{\mp 1}.
    \]
    The Nenciu data for this Hopf algebra is $s=2$, $\mb{m} = (4, 4)$ and $t = t_1+t_2$. Then $\mb{d}$and $\mb{u}$ are $t\times 2$ matrices, such that for $k=1, \dots, t_1$ $\mb{d}_k = (1, 1)$, and  $\mb{u}_k = (1, 1)$ corresponding to $X_k$. For $l=t_1+1, \dots, t_2$ the rows are $\mb{d}_{2l-1} = (1, 0)$, $\mb{u}_{2l-1} = (2, 1)$ corresponding to $Z^+_l$ and $\mb{d}_{2l} = (-1, 0)$, $\mb{u}_{2l} = (-2, -1)$ corresponding to $Z^-_l$. 
\end{example}
\noindent The minimal example occurs for $t_1 = 4$, $t_2 = 1$, and its dimension is $4\times 4 \times 2^6 = 2^{10} = 1024$. 
\begin{proposition}
    The algebra $H_1$ of Example \ref{ex1} is
    \begin{enumerate}
        \item Unimodular, with two-sided integral element (cointegral)
        \[
            \Lambda := \left(\sum^3_{a,b=0} K^a_1 K^b_2 \right) \prod^{t_1}_{k=1}X_k \prod^{t_2}_{l=1}Z^+_l
            \prod^{t_2}_{l=1}Z^-_l.
        \]
        and a two-sided integral form defined on the monomial basis by
        \[
            \lambda(\mb{X}^\mb{r} \mb{K}^\mb{v}):=
            \begin{cases}
                1 \text{\, if \,} \mb{v} = (0, 0), \mb{r} = (1, 1,\dots,1) \\
                0 \text{\, otherwise}.
            \end{cases}
        \]
        \item triangular, with the R-matrix defined for the grouplike elements 
        \[
            R_{\mb{z}} := \frac{1}{16}\sum_{\mb{v}, \mb{w} \in \Z^2_4} i^{-\mb{v}\mb{w}^T} \mb{K}^{\mb{w}} \otimes \mb{K}^{\mb{v} \mb{z}}, 
        \]
        where $\mb = (K_1, K_2)$, $\pmb{\xi} = (i, i)$, and $\mb{z} =\begin{pmatrix} 2 && 3\\ 1 &&0 \end{pmatrix}$. 
        \item and trivially ribbon, with the ribbon element $\1$, corresponding to the unique pivotal element $g = K^2_1$. 
    \end{enumerate}
\end{proposition}
\begin{remark}
    The behaviour of $Z^{\pm}$ suggests that a non-triangular R-matrix could be built of terms of the shape $Z_l^{\pm} \otimes K_1^{\pm2} K_2^{\pm1} Z_l^{\mp}$, as the two generators are of opposite type. However, any map $f_R$, sending $(Z_l^\pm)^*\mapsto K_1^{-2} K_2^{-1} (Z_l^\mp)$, satisfies all constraints bar (B1), which is equivalent to $(K_1^{2} K_2^{1})^2=\1$, which is false. Th element $X_k$ similarly fails (B1) for any map so we have no non-triangular structures.   
\end{remark}
With this observation, we can build a non-triangular example, at the cost of introducing a $K_3$, another $\Z_4$ grouplike. We can choose $L = K_3^2$, which implies that the corresponding $Z^{\pm}$ will at most anti-commute with all other nilpotents. 
\begin{example}
    \label{ex2}
    Let $H_2$ be the Hopf algebra generated by $K_a$, $X_k^{\pm}$ and $Z^{\pm}_l$, for $a=1, 2, 3$, $j, k=1, \dots, t_1$; $ t_1\in \N$ and $l, m =1, \dots, t_2$, $t_2\in \N$, subject to the following relations
    \[
        K_a^4 = \1, \;\;  \;\; K_a X^{\pm}_k = \pm i X^{\pm}_k K_a
    \]
    \[
       K_1 Z^{\pm}_l = Z^{\pm}_l K_1, \;\; K_2 Z^{\pm}_l = - Z^{\pm}_l K_2, \;\;  K_3 Z^{\pm}_l = \pm i Z^{\pm}_l K_3
    \]
    \[
        \{X^{\pm}_j, X^{\pm}_k\} = \{X^{\pm}_j, X^{\mp}_k\} = \{Z^{\pm}_l, X^{\pm}_k\} = \{Z^{\pm}_l, X^{\mp}_k\} = \{Z^{\pm}_l, Z^{\pm}_m\}=\{Z^{\pm}_l, Z^{\mp}_m\} =  0.
    \]
    Let also $L:=K_3^2$ as a shorthand, note that $L^2 = \1$. The Hopf structure is defined by
    \[
        \epsilon(K_a) = 1, \;\; \epsilon(X^{\pm}_k)=\epsilon(Z^{\pm}_l) = 0,
    \]
    \[
        \Delta(K_a) = K_a \otimes K_a, \;\; \Delta(X^{\pm}_k) = \1 \otimes X^{\pm}_k + X^{\pm}_k \otimes (K_1 K_2)^{\pm 1}, \;\; \Delta(Z^{\pm}_l) = \1 \otimes Z^{\pm}_l + Z^{\pm}_l \otimes L
    \]
    \[
       S(K_a)=K^{-1}_a \;\; S(X^{\pm}_k) = -X^{\pm}_k (K_1 K_2)^{\mp1} \;\;  S(Z^{\pm}_l) = -Z^{\pm}_l L.
    \]
    The Nenciu data for this Hopf algebra is $s=3$, $\mb{m} = (4, 4, 4)$ and $t = 2t_1+ 2t_2$. Then $\mb{d}$ and $\mb{u}$ are a $t\times 3$ matrices, such that for $k=1, \dots, t_1$ $\mb{d}_{2k-1} = (1, 1, 1)$, and  $\mb{u}_{2k-1} = (1, 1, 0)$ corresponding to $X^+_k$ and $\mb{d}_{2k} = (-1, -1, -1)$, and  $\mb{u}_{2k} = (-1, -1, 0)$ corresponding to $X^-_k$. For $l=t_1+1, \dots, t_2$ the rows are $\mb{d}_{2l-1} = (0, 2, 1)$, $\mb{u}_{2l-1} = (0,0,2)$ corresponding to $Z^+_l$ and $\mb{d}_{2l} = (0, -2, -1)$, $\mb{u}_{2l} = (0, 0, -2)$ corresponding to $Z^-_l$.
\end{example}
\noindent The minimal example occurs for $t_1 = 1$, $t_2 = 1$, and its dimension is $4\times 4\times 4 \times 2^4 = 2^{10} = 1024$. 
\begin{proposition}
    The algebra $H_2$ of Example \ref{ex2} is
    \begin{enumerate}
        \item Unimodular, with two-sided integral element (cointegral)
        \[
            \Lambda := \left(\sum^3_{a,b, c=0} K^a_1 K^b_2 K^c_3\right) \prod^{t_1}_{k=1}X^+_k \prod^{t_1}_{k=1}X^-_k \prod^{t_2}_{l=1}Z^+_l
            \prod^{t_2}_{l=1}Z^-_l.
        \]
        and a two-sided integral form defined on the monomial basis as
        \[
            \lambda(\mb{X}^\mb{r} \mb{K}^\mb{v}):=
            \begin{cases}
                1 \text{\, if \,} \mb{v} = (0, 0, 0), \mb{r} = (1, 1,\dots,1) \\
                0 \text{\, otherwise}.
            \end{cases}
        \]

        \item quasitriangular, with the R-matrix defined for the grouplike elements 
        \[
            R_{\mb{z}} := \frac{1}{64}\sum_{\mb{v}, \mb{w} \in \Z^3_4} i^{-\mb{v}\mb{w}^T} \mb{K}^{\mb{w}} \otimes \mb{K}^{\mb{v} \mb{z}}, 
        \]
        where $\mb{K} = (K_1, K_2, K_3)$ and $\mb{z} =\begin{pmatrix} 0 && 3 && 2 \\ 1 && 0 && 0 \\ 2 && 0 && 2  \end{pmatrix}$ 
        \\The skew-primitive part is 
        \[
            R_{\pmb{\alpha}} := \exp\left(\sum^{t_2}_{l = 1} \alpha_l( Z^+_l \otimes L Z^-_l - Z^-_l \otimes L Z^+_l)\right)
        \]
        for some $\pmb{\alpha}=(\alpha_1, \dots, \alpha_{t_2}) \in \C^{2t_2}$, so that 
        \[
            R_{\mb{z}} R_{\pmb{\alpha}} := \frac{1}{64}\sum_{\mb{v}, \mb{w} \in \Z^3_4} i^{-\mb{v}\mb{w}^T} \mb{K}^{\mb{w}} \otimes \mb{K}^{\mb{v} \mb{z}} \exp\left(\sum^{t_2}_{l = 1} \alpha_l( Z^+_l \otimes L Z^-_l - Z^-_l \otimes L Z^+_l)\right),
        \]
        \item ribbon, with the ribbon element
        \[
            v:= \exp \left( - 2\sum^{t_2}_{l = 0} \alpha_l Z^+_l Z^-_l  \right).
        \]
        corresponding to the pivotal element $g = L =K^2_3$, which in this example is the only such element available. 
    \end{enumerate}
\end{proposition}
\noindent If we introduce more types of variables not participating in the $R_{\pmb{\alpha}}$, say $Y^{\pm}$ we can produce more interesting commutation rules.
\begin{example}
    \label{ex3}
    Let $H_3$ be the Hopf algebra generated by $K_a$, $X_k^{\pm}$, $Y^{\pm}_k$ and $Z^{\pm}_l$, for $a=1, 2, 3$, $j, k=1, \dots, t_1$; $ t_1\in \N$ and $l, m =1, \dots, t_2$; $t_2\in \N$, subject to the following relations
    \[
        K_a^4 = \1, \;\;  \;\; K_a X^{\pm}_k = \pm i X^{\pm}_k K_a, 
    \]
    \[
       K_1 Y^{\pm}_k = \pm i Y^{\pm}_k K_1, \;\; K_2 Y^{\pm}_k = Y^{\pm}_k K_2, \;\;  K_3 Y^{\pm}_k = \pm i Y^{\pm}_l K_3
    \]
    \[
       K_1 Z^{\pm}_l = Z^{\pm}_l K_1, \;\; K_2 Z^{\pm}_l = -Z^{\pm}_l K_2, \;\;  K_3 Z^{\pm}_l = \pm i Z^{\pm}_l K_3
    \]
    \[
         \{X^{\pm}_j, X^{\pm}_k\} = \{X^{\pm}_j, X^{\mp}_k\} =  \{Y^{\pm}_j, Y^{\pm}_k\} = \{Y^{\pm}_j, Y^{\mp}_k\}, \;\; X_j Y_k = i Y_k X_j
    \]
    \[
       \{Z^{\pm}_l, X^{\pm}_k\} = \{Z^{\pm}_l, X^{\mp}_k\} = \{Z^{\pm}_l, Y^{\pm}_k\} = \{Z^{\pm}_l, Y^{\mp}_k\} = \{Z^{\pm}_l, Z^{\pm}_m\}=\{Z^{\pm}_l, Z^{\mp}_m\} =  0.
    \]
    Let also $L:=K_3^2$ as a shorthand, note that $L^2 = \1$. The Hopf structure is defined by
    \[
        \epsilon(K_a) = 1, \;\; \epsilon(X^{\pm}_k)= \epsilon(Y^{\pm}_k)=\epsilon(Z^{\pm}_l) = 0, 
    \]
    \[
        \Delta(K_a) = K_a \otimes K_a, \;\; \Delta(X^{\pm}_k) = \1 \otimes X^{\pm}_k + X^{\pm}_k \otimes (K_1 K_2)^{\pm},
    \]
    \[
         \Delta(Y^{\pm}_k) = \1 \otimes Y^{\pm}_k + Y^{\pm}_k \otimes (K_1 K^2_2)^{\pm1} \;\; \Delta(Z^{\pm}_l) = \1 \otimes Z^{\pm}_l + Z^{\pm}_l \otimes L
    \]
    \[
       S(K_a)=K^{-1}_a \;\; S(X^{\pm}_k) = -X^{\pm}_k (K_1 K_2)^{\mp1}, \;\; S(Y^{\pm}_k) = -Y^{\pm}_k (K^2_1 K_2)^{\mp1} \;\;  S(Z^{\pm}_l) = -Z^{\pm}_l L.
    \]
    The Nenciu data for this Hopf algebra is $s=3$, $\mb{m} = (4, 4, 4)$ and $t = 4t_1+ 2t_2$. Then $\mb{d}$ and $\mb{u}$ are $t\times 3$ matrices, such that for $j=1, \dots, t_1$ $\mb{d}_{2j-1} = (1, 1, 1)$, and  $\mb{u}_{2j-1} = (1, 1, 0)$ corresponding to $X^+_j$ and $\mb{d}_{2j} = (-1, -1, -1)$, and  $\mb{u}_{2j} = (-1, -1, 0)$ corresponding to $X^-_j$. 
    For $k=t_1+1, \dots, 2t_1$, $\mb{d}_{2k-1} = (1, 0, 1)$, and  $\mb{u}_{2j-1} = (2, 1, 0)$ corresponding to $Y^+_k$ and $\mb{d}_{2k} = (-1, -0, -1)$, and  $\mb{u}_{2k} = (-2, -1, 0)$ corresponding to $Y^-_k$.
    For $l=2t_1+1, \dots, t_2$ the rows are $\mb{d}_{2l-1} = (0, 2, 1)$, $\mb{u}_{2l-1} = (0,0,2)$ corresponding to $Z^+_l$ and $\mb{d}_{2l} = (0, -2, -1)$, $\mb{u}_{2l} = (0, 0, -2)$ corresponding to $Z^-_l$.
    % The commutation data for this Hopf algebra is $\mb{d}_{X^\pm} = \pm(1, 1, 1)$, $\mb{u}_{X^{\pm}} = \pm(1, 1, 0)$, $\mb{d}_{Y^\pm} = \pm(1, 0, 1)$, $\mb{u}_{Y^{\pm}} = \pm(2, 1, 0)$, $\mb{d}_{Z^{\pm}} = \pm (0, 2, 1)$, $\mb{u}_{Z^{\pm}} = \pm(0,0,2)$.
\end{example}
\noindent The minimal example occurs for $t_1 = 1$, $t_2 = 1$, and its dimension is $4\times 4\times 4 \times 2^6 = 2^{12} = 4096$.
\begin{proposition}
    The algebra $H_3$ of Example \ref{ex3} is
    \begin{enumerate}
        \item Unimodular, with two-sided integral element (cointegral)
        \[
            \Lambda := \left(\sum^3_{a,b, c=0} K^a_1 K^b_2 K^c_3 \right) \prod^{t_1}_{k=1}X^+_k \prod^{t_1}_{k=1}X^-_k 
            \prod^{t_1}_{k=1}Y^+_k \prod^{t_1}_{k=1}Y^-_k 
            \prod^{t_2}_{l=1}Z^+_l
            \prod^{t_2}_{l=1}Z^-_l.
        \]
        and a two-sided integral form defined on the monomial basis by
        \[
            \lambda(\mb{X}^\mb{r} \mb{K}^\mb{v}):=
            \begin{cases}
                1 \text{\, if \,} \mb{v} = (0, 0,  0), \mb{r} = (1, 1,\dots,1) \\
                0 \text{\, otherwise}.
            \end{cases}
        \]
            
        
        \item quasitriangular, with the R-matrix defined for the grouplike elements 
        \[
            R_z := \frac{1}{64}\sum_{\mb{v}, \mb{w} \in \Z^3_4} i^{-\mb{v}\mb{w}^T} \mb{K}^{\mb{w}} \otimes \mb{K}^{\mb{v} \mb{z}}, 
        \]
        where $\mb{K} = (K_1, K_2, K_3)$ and $\mb{z} =\begin{pmatrix} 0 && 3 && 2 \\ 1 && 0 && 0 \\ 2 && 0 && 2  \end{pmatrix}$ 
        \\The skew-primitive part is 
        \[
            R_{\pmb{\alpha}} := \exp\left(\sum^{t_2}_{l = 1} \alpha_l( Z^+_l \otimes L Z^-_l - Z^-_l \otimes L Z^+_l)\right)
        \]
        for some $\pmb{\alpha}=(\alpha_1, \dots, \alpha_{t_2}) \in \C^{2t_2}$, so that 
        \[
            R_z R_{\pmb{\alpha}} := \frac{1}{64}\sum_{\mb{v}, \mb{w} \in \Z^3_4} i^{-\mb{v}\mb{w}^T} \mb{K}^{\mb{w}} \otimes \mb{K}^{\mb{v} \mb{z}} \exp\left(\sum^{t_2}_{l = 1} \alpha_l( Z^+_l \otimes L Z^-_l - Z^-_l \otimes L Z^+_l)\right),
        \]
        \item ribbon, with the ribbon element
        \[
            v:= \exp \left( -2 \sum^{t_2}_{k = 1} \alpha_l Z^+_l Z^-_l  \right).
        \]
        corresponding to the unique pivotal element $g = L = K^2_3$. 
    \end{enumerate}
\end{proposition}

\begin{definition}
\label{SNFdef}
    We call a quasitriangular Hopf algebra $(H, R)$ \textit{strongly non-factorizable}, if for the monodromy matrix $M:= R_{21}R$ in the usual notation we have 
    \[
        (\lambda \otimes \mathrm{Id}) M = (\mathrm{Id}\otimes \lambda) M = 0.  
    \]
\end{definition}
Note that any fully-degenerate, for instance triangular such as Example \ref{ex1}, Hopf algebra is also strongly non-factorizable according to this definition. However, Examples \ref{ex2}, \ref{ex3} are both strongly non-factorizable, yet not fully degenerate, as we now show.
\begin{proposition}
\label{ExAreSNF}
    The Hopf algebras of examples \ref{ex1}, \ref{ex2}, \ref{ex3} are strongly non-factorizable.
\end{proposition}
\begin{proof}
We note that examples are in fact self-dual, that is the duality is an isomorphism of Hopf algebras, as per the assumptions of theorem \ref{R-matrixConstr}, so we can consider any $f:H^*\rightarrow H^{cop}$ to be in fact $f':H\rightarrow H^{cop}$ by precomposing $f$ with the duality. We firstly explain why the generators $X^\pm_k$ (or equally $Y^\pm_k$ for Example \ref{ex3}, we will keep using Example \ref{ex2} in this argument) cannot participate in $R_\alpha$. We see from (B1) and (C1), and a simple check of all cases that the only way to satisfy $\mb{d}_j\mb{z} = -\mb{u}_l$ is to map either $f'(X_k^\pm) = (K_1K_2)^{\mp1} X_k^\pm$, (respectively $K^2_1 K_2$ for $Y^\pm_k$ henceforth). The mapping $f'(X_k^\pm) = (K_1K_2)^{\pm 1} X_k^\mp$ analogous to the image of $Z_l^\pm$ satisfies (B1) only if $(K_1K_2) = (K_1K_2)^{-1}$, which is not the case for, any other choice of generators (i.e. image involving $Z^\pm_l$) breaks (B1) as well, which can be checked directly. Moreover, the mapping $f'(X_k^\pm) = (K_1K_2)^{\mp1} X_k^\pm$ fails (C4) for all $K_a$, $a=1, \dots, s$.
\\ Now, from the definitions of the integral and the R-matrix, it is easy to see that all nilpotent generators except $Z^\pm_l$ (or all in Example \ref{ex1}) are absent from the respective R-matrices. There is no relation available that introduces them, as the commutations are necessarily diagonal, thus they are absent from the monodromy matrix as well. Since the integral form is non-zero only on the top element, which has to contain all nilpotent generators, hence we deduce the result. 
\end{proof}


==> factorizingInvariant.tex <==
\section{The invariant corresponding to $U\ltimes H$}
In this section we show that the invariant obtained with the bead algorithm from the Hopf algebra $U \ltimes H$, $J_{U\ltimes H}$ for any 0-to-0 morphism is the product of $J_U$ and $J_H$. \\
Consider the Hopf algebra maps $j:U \ltimes H \rightarrow U$ and $p:U \ltimes H \rightarrow H$ from Remark \ref{SESproposition}. Let $\underline{U}$, $\underline{H}$ and $\underline{U \ltimes H}$, denote the \textit{transmuted Hopf algebras}, as defined in Section 7.2 of \cite{beliakova_derenzi_2023}. It is, in particular, the Hopf algebra $H$ seen as a module under the adjoint action of Definition \ref{adjointAct} on itself. By the discussion in Section 8, the bead algorithm \ref{beadalgo} is equivalent to computing the invariant from the transmuted Hopf algebra. We wish to show that there exists direct summand $\underline{\mathcal{F}}$ of $\underline{U\ltimes H}$ such that the integral $\lambda$ factorizes through $\underline{\mathcal{F}}$ as a linear map without changing the value of the invariant $J_{U\ltimes H}$. Moreover, there are direct summands $\mathcal{T} \subset \underline{H}$ and  $\mathcal{E} \subset \underline{U}$ with the same property for respective invariants $J_H$ and $J_U$, and $\underline{\mathcal{F}} \cong j^*(\mathcal{E}) \otimes p^*(\mathcal{T})$. The functors $j^*$ and $p^*$ come from the following standard fact.
\begin{proposition}
\label{pullbackProp}
    The Hopf (in particular algebra) maps 
    \[
        U \xleftarrow{j} U \ltimes H \xrightarrow{p} H
    \]
    induce the functors between the categories of modules 
    \[
        U\operatorname{-mod} \xrightarrow{j^*} (U\ltimes H)\operatorname{-mod} \xleftarrow{p^*} H\operatorname{-mod},
    \]
    where the pullback action of an $s \in U \ltimes H$ is defined for $u\in \mathcal{U} \in U\operatorname{-mod}$ and $h\in \mathcal{H} \in H\operatorname{-mod}$ is
    \begin{align*}
        s \cdot j^*(u):= j(s) \cdot_{\mathcal{U}} u, && s \cdot p^*(h):= p(s) \cdot_{\mathcal{H}} h,
    \end{align*}
\end{proposition}
\noindent In particular, the functors $j^*, p^*$ preserve direct products of modules.
\begin{definition}
    Let $\mathcal{T} \in H\operatorname{-mod}$ be the submodule of $\underline{H}$ generated by the top element $T\in \underline{H}$ under the adjoint action 
\[
    \mathcal{T}:= H\rhd \langle T \rangle 
\]
\end{definition}
\begin{proposition}
\label{Proposition:TisDirect}
    It was shown in THE OTHER PAPER that it is a direct summand of $\underline{H}$. 
\end{proposition}
\noindent Let $q_{\mathcal{T}}: \underline{H} \rightarrow \mathcal{T}$ be the corresponding quotient map. Clearly $q_{\mathcal{T}}(T)\neq 0$.\\
We can show that under the adjoint action $\underline{U}$ splits into the submodules generated by \textit{even} and \textit{odd} monomials with respect to the parity $|E^a F^b K^c| := a+c \mod 2$, for any $a, b, c \in \Z_{r'}$.
\begin{proposition}
\label{paritySplit}
    We have
\[
    \underline{U} = \mathcal{E} \oplus \mathcal{O}
\]
as $U$-modules, where
\[
    \mathcal{E}:= U \rhd \langle E^a F^b K^c, \; a, b, c\in \Z_{r'}|a+c \equiv 0 \mod 2 \rangle
\]
and
\[
    \mathcal{O}:= U \rhd \langle E^a F^b K^c, \; a, b, c\in \Z_{r'}|a+c \equiv 1 \mod 2 \rangle.
\]
\end{proposition}
\noindent In the proof we will use the following identities.
\begin{lemma}[\cite{kassel_2012}, Lemma VI.1.3]
\label{commLemma}
For $m\in \Z_{r'}$
\[
    [F^m, E] = [m] F^{m-1} \frac{q^{m-1}K^{-1}-q^{-(m-1)}K}{q-q^{-1}}
\]
and 
\[
    [E^m, F] = [m]E^{m-1}\frac{q^{(m-1)}K-q^{-(m-1)}K^{-1} }{q-q^{-1}}.
\]
    
\end{lemma}
\begin{proof}[Proof of Proposition \ref{paritySplit}]
     As defined, $\mathcal{E}$ and $\mathcal{O}$ are clearly submodules of $\underline{U}$, and $\mathcal{E} + \mathcal{O} = \underline{H}$ since the sum contains every element of the monomial basis, $E^a F^b K^c$, for $a, b, c \in \Z_{r'}$. To show that the sum, is direct, we need that $\mathcal{E} \cap \mathcal{O} = 0$, and we do this on the monomial basis. By associativity of the adjoint action, it is enough to show that the action of $E, F, K$ on any $E^a F^b K^c$ preserves the parity. Indeed first of all
     \[
        K\rhd E^a F^b K^c = q^{2(a-b)} E^a F^b K^c,
     \]
     so obviously the parity if preserved.
     Next, using the Lemma \ref{commLemma}
     \begin{align*}
         E\rhd E^a F^b K^c & = - E^a F^b K^c E K + E E^a F^b K^c K^{-1} \\
         = & - q^{2}E^a F^b E K^{c+1} + E^{a+1} F^b K^{c-1} \\
         = & - q^{2}E^{a+1} F^b  K^{c+1} - q^{2}[b] E^a F^{b-1} \frac{q^{b-1}K^{-1}-q^{-(b-1)}K}{q-q^{-1}} K^{c+1} \\
           &+ E^{a+1} F^b K^{c-1},
     \end{align*}
      and we see the parity is preserved in each summand, as the exponent of $F$ is irrelevant. Similarly,
      \begin{align*}
          F\rhd E^a F^b K^c & = F E^a F^b K^{c} - K^{-1} E^a F^b K^{c} F K\\
          = & F E^a F^b K^{c} - q^{2(-a+b-c+1)} E^a F^{b+1} K^{c}  \\
          = & [a]E^{a-1}\frac{q^{(a-1)}K-q^{-(a-1)}K^{-1} }{q-q^{-1}} F^b K^{c} + E^a F^{b+1} K^{c}\\
          &- q^{2(a-b-c-1)} E^a F^{b+1} K^{c+1},
      \end{align*}
      so again the parity is preserved. Hence, since the generating sets of $\mathcal{E}$ and $\mathcal{O}$ are disjoint, consisting of monomials of opposite parity, and the adjoint action preserves parity we have $\mathcal{E} \cap \mathcal{O} = 0$ as desired.
\end{proof}
\noindent Let $q_{\mathcal{E}}: \underline{U} \rightarrow \mathcal{E}$ be the corresponding quotient map. 
Clearly, $q_{\mathcal{E}}(E^{r'-1}F^{r'-1}K^{r'-1})$ is non-zero.
\begin{definition}
Define the module $\mathcal{F} \in (U \ltimes H) \operatorname{-mod}$ to be
\[
    \mathcal{F} := j^*(\mathcal{E})\otimes p^*(\mathcal{T}).
\]
\end{definition}
\begin{definition}
Define also the following submodules of $\underline{U\ltimes H}$
\begin{align*}
    \underline{\mathcal{T}}&:= (U\ltimes H) \rhd \mb{X}^{(1, \dots, 1)}\\
    \underline{\mathcal{E}}&:=U\ltimes H \rhd \langle E^a F^b K^c, \; a, b, c\in \Z_{r'}|a+c \equiv 1 \mod 2 \rangle\\
    \underline{\mathcal{F}}&:=U\ltimes H \rhd \langle E^a F^b K^c \mb{X}^{(1, \dots, 1)}, \; a, b, c\in \Z_{r'}|a+c \equiv 1 \mod 2 \rangle
\end{align*}
\end{definition}
We prove first the following.
\begin{lemma}
    The submodules $\underline{\mathcal{T}}$ and $\underline{\mathcal{E}}$ are direct summands of $\underline{U\ltimes H}$.
\end{lemma}
\begin{proof}
    We have to prove no $\underline{\mathcal{T}}$ and $\underline{\mathcal{E}}$ intersect no other submodules of $\underline{U\ltimes H}$ that are not submodules of $\underline{\mathcal{T}}$ and $\underline{\mathcal{E}}$, respectively. As in Proposition \ref{paritySplit}, the result for $\underline{\mathcal{T}}$ is analogous to THE OTHER PAPER applied to $E$ and $F$. For $\underline{\mathcal{E}}$, let $\underline{\mathcal{M}}\subset \underline{U\ltimes H}$ be any such submodule. We know from Proposition \ref{Proposition:TisDirect} that if any element $u\in \underline{\mathcal{M}}$, containing only generators $E, F, K$, then $|g|=0$. If we call $$\underline{\mathcal{M}}_0 := \{u\in \underline{\mathcal{M}}| |u|=0, \; \textbf{generated by only } E, F, K\}$$ containing only such elements, then it has to be a direct summand of $\underline{\mathcal{M}}$, by the same argument as in Proposition \ref{Proposition:TisDirect}. We now just need to show that for no element $h \in \underline{\mathcal{M}}$ generated by $K_a, X_k$ and even elements generated by $E, F, K$ by the diagonality of relations. Let $h = \mb{K}^{\mb{v}}\mb{X}^{\mb{r}}$ for $\mb{v}\in \Z_\mb{m}$ and $\mb{r} \in \Z^t_2$. Then we know immediately that $K\rhd \mb{K}^{\mb{v}}\mb{X}^{\mb{r}} = (-1)^{|\mb{X}^{\mb{r}}|} \mb{K}^{\mb{v}}\mb{X}^{\mb{r}}$ and $F\rhd \mb{K}^{\mb{v}}\mb{X}^{\mb{r}} = 0$. Moreover
    \[
        E \rhd \mb{K}^{\mb{v}}\mb{X}^{\mb{r}} = -2 \mb{K}^{\mb{v}}\mb{X}^{\mb{r}} EK^{-1} \text{ if } |\mb{K}^{\mb{v}}\mb{X}^{\mb{r}}| = 1
    \]
    and 0 otherwise. Hence, no such element can belong to $\underline{\mathcal{E}}$. Hence $\underline{\mathcal{E}}$ is a direct summand of $\underline{U\ltimes H}$.  
\end{proof}
\begin{lemma}
    The maps 
    \begin{align*}
        \mathcal{T} &\xrightarrow{p^*} \underline{\mathcal{T}} \\
        \mathcal{E} &\xrightarrow{j^*} \underline{\mathcal{E}}
    \end{align*}
are isomorphisms of $(U \ltimes H)$-modules, where $\mathcal{T}$ is considered a module where the $U$ piece acts trivially and $H$ piece adjointly, and $\mathcal{E}$ one where $H$ piece acts trivially and $U$ piece adjointly.
\end{lemma}
\begin{proof}
    The explicit assignments on the momnomial bases are, reestablishing the internal tensor product of $U\ltimes H$  
    \begin{align*}
        X^{(1, \dots, 1)} &\xmapsto{p^*} \1_U \otimes X^{(1, \dots, 1)}\\
        E^a F^b K^c & \xmapsto{j^*} E^a F^b K^c \otimes \1_H, 
    \end{align*}
    so a direct comparison of the actins is enought to establish isomorphisms.
\end{proof}
\begin{lemma}
\label{ETF}
    We have the isomorphism of $U\ltimes H$ modules
    \[
        \underline{\mathcal{E}} \otimes \underline{\mathcal{T}} \cong \underline{\mathcal{F}}.
    \]
\end{lemma}
\begin{proof}
We have the obvious map on the monomial bases
\begin{align*}
    f:\underline{\mathcal{E}} \otimes \underline{\mathcal{T}} &\rightarrow \underline{\mathcal{F}}\\
    E^a F^b K^c \otimes \mb{X}^{(1, \dots, 1)} &\mapsto E^a F^b K^c \mb{X}^{(1, \dots, 1)},
\end{align*}
so it is left to compare the actions. By Propositions \ref{Proposition:TisDirect}, \ref{paritySplit} we know the action on $\underline{\mathcal{E}} \otimes \underline{\mathcal{T}}$ is such that $\underline{\mathcal{T}}$ is acted upon only by the $U$ piece and $\underline{\mathcal{E}}$ only by the $H$ piece. On the other hand, we have the action on $\underline{\mathcal{F}}$, for $u \in \{E, F, K\}$ and $h\in \{K_a, X_k\}$
    \begin{align*}
        u \rhd E^a F^b K^c \mb{X}^{(1, \dots, 1)} &= (u \rhd E^a F^b K^c) \mb{X}^{(1, \dots, 1)}\\
        h \rhd E^a F^b K^c \mb{X}^{(1, \dots, 1)} &= E^a F^b K^c (h\rhd \mb{X}^{(1, \dots, 1)})
    \end{align*}
as $\mb{X}^{(1, \dots, 1)}$ is central and $|E^a F^b K^c|=1$.
\end{proof}
% \begin{remark}
% \label{FRemark}
% It can be shown that 
% \[
%     \mathcal{F}\cong U\ltimes H \rhd \langle E^a F^b K^c \mb{X}^{(1, \dots, 1)}, \; a, b, c\in \Z_{r'}|a+c \equiv 1 \mod 2 \rangle \subset \underline{U\ltimes H},
% \]
% \end{remark}
Thus we can deduce two facts.
\begin{corollary}
\label{FisDirect}
    The module $\underline{\mathcal{F}}$ is a direct summand of $\underline{U\ltimes H}$ under adjoint action.
\end{corollary}
\begin{proof}
    This follows from Lemma \ref{ETF} and the fact that tensor product is distributive over direct sums.
\end{proof}
\begin{corollary}
\label{Ffactorizes}
    We have the isomorphism of $U\ltimes H$-modules
    \[
        p^*(\mathcal{E}) \otimes j^*(\mathcal{T}) \cong \underline{\mathcal{F}}.
    \] 
\end{corollary}

% \begin{proposition}
%     The module $\mathcal{F}$ is a direct summand of $\underline{U \ltimes H}$ under the adjoint action.
% \end{proposition}
% \begin{proof}
% %Maybe better to shown E and T are direct summands in U \ltimes H, which is lamost immediate, because the cross-actions are trivial. Then the tensor still has the decoupled action so is gonna be a direct summand as well.
%      %The adjoint action of all elements preserves the parity of $E^a F^b K^c$ and $T$ is central. 
%      We first remark that $\mathcal{F}$ is a tensor product of $(U \ltimes H)$-modules, and thus we consider the action of $(U \ltimes H)$ via the coproduct. In conformity with the notation of Proposition \ref{pullbackProp}, let $u^*:=j^*(u)\in j^*(\mathcal{E})$ and $T^*:=p^*(T)\in p^*(\mathcal{T})$, where the latter is associated with the top element of $H$, which generates the module, we drop any constant prefactors for the sake of the argument. We have explicitly, denoting the action of $U\ltimes H$ with a dot
%      \begin{align*}
%          \Delta(K_a) \cdot (u^* \otimes T^*) =& u \otimes (K_a \rhd T) = u \otimes T\\
%          \Delta(X_k) \cdot (u^* \otimes T^*) =& u \otimes (X_k \rhd T)=0\\
%          \Delta(K) \cdot (u^* \otimes T^*) =& (K \rhd u) \otimes (K \rhd T) = (E \rhd u) \otimes T\\
%          \Delta(E) \cdot (u^* \otimes T^*) =& (E \rhd u) \otimes (K \rhd T) = (E \rhd u) \otimes T\\
%          \Delta(F) \cdot (u^* \otimes T^*) =& (F \rhd u) \otimes T.   
%      \end{align*}
%      Thus, the actions of $U$ and $H$ decouple, and this is exactly the action on the module $\underline{\mathcal{T}} \otimes \underline{\mathcal{E}} \cong \underline{\mathcal{F}}$. Thus, the map
%      \[
%         \mathcal{F} \xrightarrow{j^*\otimes p^*} \underline{\mathcal{F}}
%      \]
%      is an isormophism and we established that $\mathcal{F}$ is a submodule of $\underline{U\ltimes H}$. Now we show it is a direct summand. But it is a tensor product of two direct summands with the action factorizing, so indeed it is.
%      %It is now left to show that is does not intersect any other submodules $Q\subset \underline{U\ltimes H}$. This is tantamaount to showing that there exists no $s\in \underline{U \ltimes H}$ such that the submodule $\mathcal{S}:=(U \ltimes H)\rhd s$ has $\mathcal{S} \cap \mathcal{F}=0$. Firstly, we can read from the above that the adjoint action preserves the parity of the $U$-piece, thus by the same argument as for Proposition \ref{paritySplit}, any such $s$ needs to have a definite positive parity in $E, F, K$. Thus, we can assume $s$ is a monomial, say $E^a F^b K^c \mb{K}^\mb{v}\mb{X}^\mb{r}$ for $a+c\equiv 0 \mod 2$, $\mb{v} \in \Z_\mb{m}$ and $\mb{r}\in \Z^t_2$. Since $E^a F^b K^c$ by parity commutes with any $K_a$, $X_k$ the adjoint action of the generators has the form
%      %  \[
%      %    K_a \rhd E^a F^b K^c \mb{K}^\mb{v}\mb{X}^\mb{r} = E^a F^b K^c(K_a \rhd \mb{K}^\mb{v}\mb{X}^\mb{r})
%      %  \]
%      %  \[
%      %    X_k \rhd E^a F^b K^c \mb{K}^\mb{v}\mb{X}^\mb{r} = E^a F^b K^c(X_k \rhd \mb{K}^\mb{v}\mb{X}^\mb{r}).
%      %  \]
%      %  Now we can invoke the argument of THE OTHER PAPER, that $T$ cannot be reached from any monomial this way. Hence $s \in \mathcal{F}$, and the sum is direct.
% \end{proof}
\noindent Let the corresponding quotient map be $q_\mathcal{F}: U \ltimes H \rightarrow \underline{\mathcal{F}}$. Clearly, $q_{\underline{\mathcal{F}}}(E^{r'-1}F^{r'-1}K^{r'-1}T) \neq 0$.
% \begin{remark}
%     Any modules can be used as long as the top elements are preserved and the last property holds.
% \end{remark}
\begin{remark}
    Because the modules are direct summands, we can speak of the images of the top elements as indeed copies of them.
\end{remark}
\begin{definition}
    We define the maps $\Bar{J}_H$, $\Bar{J}_U$, $\Bar{J}_{U\ltimes H}$, which differ from the invariant by precomposing $\lambda_{H} \circ q_\mathcal{T}$, $\lambda_{U} \circ q_\mathcal{E}$ and $\lambda_{U\ltimes H} \circ q_{\underline{\mathcal{F}}}$. 
\end{definition}
\begin{proposition}
\label{JBar}
    For any 0-0 morphism $W$ of $\mb{4HB}$, we have
    \begin{align*}
        \Bar{J}_H(W) = J_H(W) && \Bar{J}_U(W) = J_U(W) && \Bar{J}_{U\ltimes H}(W) = J_{U\ltimes H}(W).
    \end{align*}
\end{proposition}
\begin{proof}
    We know the integrals $\lambda_{U}$ $\lambda_{H}$ $\lambda_{U\ltimes H}$ are non-zero only for the elements $E^{r'}F^{r'}K^{r'} \in U$, $\mb{X}^{(1, \dots, 1)}\in H$ and $E^{r'}F^{r'}K^{r'}\mb{X}^{(1, \dots, 1)} \in U\ltimes H$. By Propositions \ref{paritySplit}, \ref{Proposition:TisDirect} and Corollary \ref{FisDirect} and commentary beneath them, the elements are preserved by the maps $q_\mathcal{E}$, $q_\mathcal{T}$ and $q_{\underline{\mathcal{F}}}$ respectively. \\
    In the final step of the bead algorithm \ref{beadalgo}, the integrals of the Hopf algebra $A$ are applied to the element carried by the bead on each 2-handle. By Section 8 of \cite{beliakova_derenzi_2023}, the beads collectively give an element of $\underline{A}^{\otimes k_2}$, where $k_2$ is the number of 2-handles in the diagram of $W$. We apply $\lambda_A^{\otimes k_2}$ to that element and again pick only the summand containing $T^{\otimes k_2}$ where $T \in A$ is the only monomial picked up by $\lambda_A$, we call the \textit{top element}.\\
    Let now $A\in \{U, H, U\ltimes H\}$. We see that this top element is is preserved by the respective quotient map. Thus, the value of the maps $\Bar{J}_A$ is the same as $J_A$. 
\end{proof}
\begin{proposition}
Let $W$ be a 0-0 morphism of \textbf{4HB}. Then 
    \[
        \Bar{J}_{U\ltimes H}(W) = \Bar{J}_{U}(W)\Bar{J}_{H}(W)
    \]
    so by Proposition\ref{JBar}
    \[
        J_{U\ltimes H} = J_{U}(W)J_{H}(W).
    \]
\end{proposition}
\begin{proof}
     % Let $W$ be a 0-0 morphism of \textbf{4HB}. We fix the corresponding Kirby diagram, as what follows is independent of this choice. Now, as in the preceeding proposition, we perform all steps of the bead algorithm \ref{beadalgo} except for the final application of the integrals, which should become apparent. The result is an element of $(\underline{U\ltimes H})^{\otimes k_2}$, where $k_2$ is the number of 2-handles in the fixed diagram of $W$, and can be written generally schematically as 
     % \begin{align*}
     %     \mathcal{J} =& \sum_{\mb{i} \in \Z_{\dim(U \ltimes H)}^{k_2}} \alpha_{\mb{i}} x_{i_1}\otimes \dots \otimes x_{i_2}\\
     %     =& \alpha_{(1, \dots, 1)} \1\otimes \dots \otimes \1 + \dots +  \alpha_{(\dim(U \ltimes H), \dots, \dim(U \ltimes H))} E^{r'-1}F^{r'-1}K^{r'-1} \mb{X}^{(1, \dots, 1)}\otimes \dots \otimes E^{r'-1}F^{r'-1}K^{r'-1} \mb{X}^{(1, \dots, 1)}
     % \end{align*}
     % where each $\alpha_{\mb{i}} \in \C$ are constants an each $x_{i_j}$ is a monomial in $U\ltimes H$. Clearly, $\alpha_{(\dim(U \ltimes H), \dots, \dim(U \ltimes H))}=J_{U\ltimes H}$, as  $\lambda_{U\ltimes H}(E^{r'-1}F^{r'-1}K^{r'-1} \mb{X}^{(1, \dots, 1)})=1$, and since $J_{U\ltimes H}(W)$ is an invariant of $W$ this value is independent of the choice of the diagram. Since $E^{r'-1}F^{r'-1}K^{r'-1} \mb{X}^{(1, \dots, 1)}) \in \mathcal{F}$, and moreover $q_{\mathcal{F}}(E^{r'-1}F^{r'-1}K^{r'-1} \mb{X}^{(1, \dots, 1)}))=E^{r'-1}F^{r'-1}K^{r'-1} \mb{X}^{(1, \dots, 1)})\in \mathcal{F}$, so the value of $$ 
In this proposition we will restore the internal tensor product of $U\ltimes H$, in particular we will denote the monomials therein by $E^a F^b K^c \otimes \mb{K}^\mb{v}\mb{X}^\mb{r}$. The reason for this is that from Theorem \ref{extMainThm} we have that $\lambda_{U\ltimes H}:= \lambda_{U} \otimes \lambda_{H}$. 
For $(\underline{U\ltimes H})^{\otimes k_2}$ the integral picks up only the element $\alpha_{U\ltimes H} (E^{r'}F^{r'}K^{r'} \otimes \mb{X}^{(1, \dots, 1)})^{\otimes k_2}$ for $\alpha_{U\ltimes H} \in \C$. So we find
\[
        J_{U\ltimes H}(W) = \alpha_{U\ltimes H} \lambda^{\otimes k_2}_{U\ltimes H}((E^{r'}F^{r'}K^{r'}\otimes\mb{X}^{(1, \dots, 1)})^{k_2}) = \alpha_{U\ltimes H}\lambda_U(E^{r'}F^{r'}K^{r'})^{\otimes k_2} \lambda_H (\mb{X}^{(1, \dots, 1)})^{k_2}.
\]
where the second equality follows from the definition of $\lambda_{U\ltimes H}$. Now we repeat the reasoning for $U$ and $H$. Let the top elements of $U$ and $H$ in the computation of $J_U$ and $J_H$, be $\alpha_U E^{r'-1} F^{r'-1} K^{r'-1}$ and $\alpha_H \mb{X}^{(1, \dots, 1)}$, respectively. Then 
\begin{align*}
    J_{U}(W) &= \alpha_{U} \lambda^{\otimes k_2}_{U}(E^{r'-1}F^{r'-1}K^{r'-1})\\
    J_{H}(W) &= \alpha_{H} \lambda^{\otimes k_2}_{H}(\mb{X}^\mb{(1, \dots, 1)})
\end{align*}
\textcolor{red}{Problem}: how do we show $\alpha_{U\ltimes H} = \alpha_U \alpha_H$?.



     
\end{proof}

% \begin{remark}
%     This should be enough because the integral is just a linear map. Even vector spaces would be enough, as we only use module structure to prove the direct sum.
% \end{remark}
